A critical study of the Monte Carlo replica method

We present a detailed mathematical study of the Monte Carlo replica method as applied in the global fitting literature from the high-energy physics theory community. For the first time, we provide a rigorous derivation of the parameter distributions implied by the method, and show that, whilst they agree with Bayesian posteriors for linear models, they disagree otherwise. We proceed to numerically quantify the disagreement between the Monte Carlo replica method and the Bayesian method in the context of two phenomenologically relevant scenarios: fits of the SMEFT Wilson coefficients, and fits of PDFs (albeit in a toy scenario). In both scenarios, we find that uncertainty estimates of the quantities of interest are discrepant between the two approaches when non-linearity is relevant. Our findings motivate future investigation of Bayesian methodologies for global PDF fits, especially in the context of simultaneous determination of PDFs and SMEFT Wilson coefficients.

==> app-bootstrap.tex <==
\section{The Monte Carlo replica method as a parametric bootstrap}
\label{app:parametric_bootstrap}

Let us consider Example 2 again in the context of the parametric bootstrap. This time, we start with $N$ observations of the data,
\begin{equation}
d_1, ..., d_N,
\end{equation}
instead of a single observation. We then construct a best-fit value of the parameter $c$ through minimising the $\chi^2$-statistic to the entire sample of data:
\begin{equation}
c^* := \argmin_{c} \left( \frac{(d_1 - t(c))^2}{\sigma^2} + \cdots + \frac{(d_N - t(c))^2}{\sigma^2} \right).
\end{equation}
The minimiser satisfies the quadratic equation:
\begin{equation}
t'(c)\left( \frac{d_1 + ... + d_N}{N} - t(c)\right) = 0,
\end{equation}
which has solution depending on the average data $\bar{d} = (d_1 + ... + d_N)/N$:
\begin{equation}
c^* = \begin{cases} -\displaystyle \frac{t_{\text{lin}}}{2t_{\text{quad}}} & \text{if $\bar{d} \leq t_0 - (t_{\text{lin}})^2 / 4t_{\text{quad}}$,}\\[1.5ex]
\displaystyle \frac{-t_{\text{lin}} \pm \sqrt{(t_{\text{lin}})^2 - 4 t_{\text{quad}}(t_0 - \bar{d})}}{2t_{\text{quad}}} & \text{otherwise.}\end{cases}
\end{equation}
The parametric bootstrap now proceeds to generate pseudodata samples centred on $d_0 = t(c^*)$. In particular, we generate samples of size $N$ and fit them using the minimisation of the $\chi^2$-statistic; therefore, we have:
\begin{align}
c_p(\vec{d}_p = (d_{1,p} ... , d_{N,p})) &:=\notag \argmin_{c} \left( \frac{(d_{1,p} - t(c))^2}{\sigma^2} + \cdots + \frac{(d_{N,p} - t(c))^2}{\sigma^2} \right)\\[1.5ex]
&= \begin{cases} -\displaystyle \frac{t_{\text{lin}}}{2t_{\text{quad}}} & \text{if $\bar{d}_p < t_0 - (t_{\text{lin}})^2 / 4t_{\text{quad}}$,}\\[1.5ex]
\displaystyle \frac{-t_{\text{lin}} \pm \sqrt{(t_{\text{lin}})^2 - 4 t_{\text{quad}}(t_0 - \bar{d}_p)}}{2t_{\text{quad}}} & \text{otherwise.}\end{cases}
\end{align}
In particular, the distribution of $c_p(\vec{d}_p)$ is given by:
\begin{align}
p(c) &\propto \notag\int d^N\vec{d}_p \delta\left( c - c_p(\vec{d}_p)\right) \exp\left( -\frac{1}{2\sigma^2} \left( (d_{1,p} - t(c^*))^2 + \cdots + (d_{N,p} - t(c^*))^2 \right) \right)\\[1.5ex]
&= \notag\delta\left( c + \frac{t_{\text{lin}}}{2t_{\text{quad}}} \right) \int\limits_{\bar{d}_p < t_{\text{min}}} d^N\vec{d}_p\exp\left( -\frac{1}{2\sigma^2} \left( (d_{1,p} - t(c^*))^2 + \cdots + (d_{N,p} - t(c^*))^2 \right) \right)\\
&  \qquad+ 2|2 t_{\text{quad}}c + t_{\text{lin}}| \int\limits_{\bar{d}_p > t_{\text{min}}} d^N \vec{d}_p \delta(\bar{d}_p - t(c)) \exp\left( -\frac{N}{2\sigma^2} \left( (t(c^*) - \bar{d}_p)^2 + \frac{d_{1,p}^2 + ... + d_{N,p}^2}{N} - \bar{d}_p^2 \right) \right),
\end{align}
where $t_{\text{min}} = t_0 - (t_{\text{lin}})^2/4t_{\text{quad}}$. Now, for large $N$ we have:
\begin{equation}
\bar{d}_p \approx t(c^*), \qquad \frac{d_{1,p}^2 + ... + d_{N,p}^2}{N} - \bar{d}_p^2 \approx \sigma^2,
\end{equation}
which implies that the final distribution of the pseudodata replicas approximates:
\begin{equation}
p(c) \approx 2|2t_{\text{quad}}c +t_{\text{lin}}| \exp\left( -\frac{N}{2\sigma^2} (t(c^*) - t(c))^2 \right),
\end{equation}
which can be used to obtain approximate \textit{frequentist} bounds. The result is still not equivalent to a Bayesian approach, however.

==> sec-1d.tex <==
\section{A toy example: one data point, one parameter}
\label{sec:1d}
In this section, we contrast the use of frequentist and Bayesian methods with the Monte-Carlo replica method in the context
of fitting a single theory parameter $c$, given a single data point $d$. We shall assume that our theory prediction is a (continuous) function
$t(c)$ of the single parameter $c$, and that the data is distributed normally according to:
\begin{equation}
d \sim \mathcal{N}(t(c), \sigma^2),
\end{equation}
where $\sigma^2$ is the experimental variance. In each of the methods, our aim
is to produce an \textit{interval estimate} for the parameter $c$; in the broadest possible sense, an interval estimate 
should somehow quantify the region where we expect $c$ to lie. 

There is no one standard interval estimate which is strictly `better' than others; the important thing is to understand 
the interpretation of our interval estimate once we have decided on what we are using. Two standard types arise from 
frequentist and Bayesian approaches to the problem of estimating the parameter $c$:

\begin{itemize}
\item \textbf{Confidence intervals.} In frequentist statistics, the parameter $c$ is considered fixed. A \textit{$100\alpha$\% confidence interval} for $c$ is then a \textit{random interval} $I \subseteq \mathbb{R}$, dependent on the (random) observed value of the data $d$, which contains the true value of $c$ with probability $\alpha$. In other words, if we were to repeat our experimental observation $100$ times, and construct confidence intervals from each of the observations, then approximately $100\alpha$ of our confidence intervals would contain the true value of the parameter $c$.
\item \textbf{Credible intervals.} In Bayesian statistics, the parameter $c$ is considered a random variable. We initially assume that this parameter follows some \textit{prior} probability density $\pi(c)$; this is then updated using Bayes' theorem to a \textit{posterior} probability density $p(c|d)$ given the observed data. A \textit{$100\alpha$\% credible interval} for $c$ is then an interval $I$ satisfying:
\begin{equation*}
\int\limits_{I} p(c|d)\ dc = \alpha.
\end{equation*}
That is, there is a probability $\alpha$ that our parameter lies in the interval $I$, given our prior knowledge and the observed data.
\end{itemize}

\noindent At a cursory glance, it seems that these two definitions are the same; however, it is very important to note that these two interval estimates need not coincide. We shall explicitly see this in this work, but various examples are available in the statistics literature to highlight this point (e.g. E. T. Jaynes in Ref.~\cite{}).

\subsection{Frequentist method: confidence intervals}
\label{subsec:freq1d}
Let us first derive confidence intervals for the given problem. The standard procedure for producing confidence intervals in the frequentist framework begins by identifying a \textit{pivot} random variable, whose distribution is independent of the parameter $c$ which we wish to estimate. In our case, an appropriate pivot is:
\begin{equation}
\frac{d - t(c)}{\sigma} \sim \mathcal{N}(0,1),
\end{equation}
which is distributed as a univariate normal. Now in order to construct a $100\alpha$\% confidence interval for the parameter $c$, suppose we find an interval $I \subseteq \mathbb{R}$ satisfying:
\begin{equation}
\mathbb{P}\left( \frac{d - t(c)}{\sigma} \in I \right) = \alpha.
\end{equation}
This is a straightforward task, since $(d - t(c))/\sigma$ has a known univariate normal distribution. Rearranging the inclusion inside the probability, we see that:
\begin{equation}
\mathbb{P}\left( c \in  t^{-1}(d - \sigma I)  \right) = \alpha,
\end{equation}
where $d - \sigma I = \{ d - \sigma x : x \in I\}$, and $t^{-1}$ denotes the \textit{preimage} of the theory function (rather than the inverse, which may not exist). We immediately deduce that:
\begin{equation}
t^{-1}\left(d-\sigma I\right)
\end{equation}
is a $100\alpha$\% confidence interval for $c$.\footnote{It is straightforward to show that, in fact, all confidence intervals are of this form. Note also that the continuity of $t$ ensures that this preimage is in fact an interval, given that $I$, and thus $d - \sigma I$, are intervals.
%
%Conversely, suppose that $J$ is a $100\alpha$\% confidence interval for $c$. By definition, we have $\mathbb{P}(c \in J) = \alpha$, so:
%\begin{equation}
%\mathbb{P}\left( \frac{ d - t(c) }{\sigma} \in \frac{d - t(J)}{\sigma} \right) = \alpha,
%\end{equation}
%where $(d - t(J))/\sigma = \{(d - t(x))/\sigma : x \in J\}$.
} It is customary to choose $I$ a symmetric interval about $0$; in this case, we have $I = (-z_{\alpha},z_{\alpha})$, where $z_{\alpha} \in \mathbb{R}$ is the unique value satisfying $\alpha = \Phi(z_{\alpha}) - \Phi(-z_{\alpha}) = 2\Phi(z_{\alpha}) - 1$, with $\Phi$ the cumulative distribution function of the univariate normal distribution. Then our confidence interval reduces to:
\begin{equation}
t^{-1}\left( (d -\sigma z_{\alpha}, d + \sigma z_{\alpha}) \right)
\end{equation}
If the theory $t(c)$ is sufficiently simple, we can compute confidence intervals analytically. Two interesting examples include \textit{linear} theories and \textit{quadratic} theories:

\begin{itemize}
\item \textbf{Example 1: Linear theory.} Suppose that the theory is linear, $t(c) = t_0 + t_1 c$, with $t_1 \neq 0$. Then we can invert $t$ explicitly, yielding $t^{-1}(y) = (y - t_0) / t_1$. Thus we have:
\begin{equation}
t^{-1}\left( (d -\sigma z_{\alpha}, d + \sigma z_{\alpha}) \right) = \left( \frac{d - t_0 - \sigma z_{\alpha}}{t_1}, \frac{d - t_0 + \sigma z_{\alpha}}{t_1} \right) 
\end{equation}
is a $100\alpha$\% confidence interval for $c$.

\item \textbf{Example 2: Quadratic theory.} Suppose that the theory is quadratic, $t(c) = t_0 + t_1 c + t_2 c^2$, with $t_2 \neq 0$. Now, the inverse of $t$ no longer exists, but we can still compute the preimage $t^{-1}(y) := t^{-1}(\{y\})$ given any $y \in \mathbb{R}$. We find that:
\begin{equation}
t^{-1}(y) = \begin{cases} \displaystyle \left\{\frac{-t_1 \pm \sqrt{t_1^2 - 4t_2 (t_0 - y)}}{2t_2}\right\}, &\text{if $t_1^2 \geq 4t_2(t_0 - y)$,} \\[3ex]  \emptyset, & \text{otherwise.} \end{cases}
\end{equation}
Depending on the values of $d$ and $\alpha$, this translates into the following cases for $100\alpha$\% confidence intervals:
\end{itemize}

Given more complicated functions $t(c)$, we need to work numerically instead; we defer examples of algorithms which can be applied to this problem to the multivariate generalisation given in Sect.~\ref{subsec:freqmulti}.


\subsection{Bayesian method: credible intervals}
\label{subsec:bayes1d}

In a Bayesian approach to interval estimation, we begin by assuming that before our experimental observation, our parameter $c$ is a random variable distributed according to some \textit{prior} probability density, $c \sim \pi(c)$; this is supposed to encode our existing knowledge and assumptions about the distribution of $c$, before we receive the information from the experiment. After the observation, our knowledge of the parameter's distribution is updated according to Bayes' theorem:
\begin{equation}
p(c|d) \propto \pi(c)p(d|c) = \pi(c) \exp\left( -\frac{1}{2\sigma^2} (d - t(c))^2 \right),
\end{equation}
where we assume the data is distributed according to a normal distribution $\mathcal{N}(t(c), \sigma^2)$ given the parameter $c$. The resulting density is called the \textit{posterior} probability density for $c$, and can be used to construct credible intervals as briefly alluded to in the introduction to this section; a $100\alpha$\% credible interval is an interval $I \subseteq \mathbb{R}$ such that:
\begin{equation}
N \int\limits_{I} dc\ \pi(c) \exp\left( -\frac{1}{2\sigma^2} (d - t(c))^2 \right) = \alpha,
\end{equation}
where $N$ is the appropriate normalisation of the posterior distribution.

As in the frequentist construction of confidence intervals, we are faced with many possible choices of $I$. Canonical choices for $I$ include the following:

\begin{itemize}
\item \textbf{Highest posterior density credible intervals.} In this approach, we determine the constant $p_{\alpha}$ such that:
\begin{equation}
N\int\limits_{\{c\ :\ p(c|d) > p_{\alpha}\}} dc\ \pi(c) \exp\left( -\frac{1}{2\sigma^2} (d - t(c))^2 \right) = \alpha,
\end{equation}
where $p(c|d)$ is the normalised posterior density; our credible interval is then given by $I = \{c : p(c|d) > p_{\alpha}\}$. 

\item \textbf{Equal-tailed credible intervals.} 
\end{itemize}


\noindent Given the definition of credible intervals, let us construct them for some basic examples of theory $t(c)$:

\begin{itemize}
\item \textbf{Example 1: Linear theory.} Suppose that the theory is linear, $t(c) = t_0 + t_1 c$, with $t_1 \neq 0$. Then the posterior distribution takes the form:
\begin{equation}
\pi(c) \exp\left( -\frac{1}{2\sigma^2} (d - t_0 - t_1 c)^2 \right),
\end{equation}
which is an unknown prior function $\pi(c)$ multiplied by a Gaussian. The choice of prior determines whether we can analytically determine credible intervals.

Suppose that we take $\pi(c)$ infinitesimally flat, $\pi(c) \propto 1$ (i.e. we are agnostic to any particular value of $c$ before receiving the data $d$); in this case, the posterior can be rewritten in the form:
\begin{equation}
p(c|d) \propto \exp\left( - \frac{t_1^2}{2\sigma^2} \left( c - \frac{(d - t_0)}{t_1}\right)^2 \right).
\end{equation}
Further, the highest posterior density credible intervals and equal-tailed credible intervals are analytically tractable and coincide; they are given by:
\begin{equation}
\left( \frac{d - t_0 - \sigma z_{\alpha}}{t_1}, \frac{d - t_0 + \sigma z_{\alpha}}{t_1} \right),
\end{equation}
with $z_{\alpha}$ such that $2\Phi(z_{\alpha}) - 1 = \alpha$, and $\Phi$ the cumulative distribution function of the univariate normal. This is precisely the confidence interval we obtained by the frequentist method for linear theory. In particular, we see that \textit{the frequentist and Bayesian methods agree for linear theory, in the limit where the Bayesian prior becomes flat}. However, even for linear theory, we see that the Bayesian and frequentist methods will \textit{disagree} if we take some other prior; in the Bayesian analysis, the prior is important.
\end{itemize}

\noindent Already in the case where the theory is quadratic, the Bayesian approach becomes analytically intractable (which should already raise a warning to the alert reader that the Bayesian credible intervals will not, in general, coincide with the frequentist confidence intervals). We can perform some numerical simulations to determine credible intervals in this case though...






\subsection{The Monte-Carlo replica method}
\label{subsec:mc_replica_1d}

The Monte-Carlo replica method is neither fully frequentist or fully Bayesian in its approach. In this method, given the observed data $d$ we introduce a \textit{pseudodata replica} $d_p$ as a random variable with normal distribution $\mathcal{N}(d,\sigma^2)$:
\begin{equation}
d_p \sim \mathcal{N}(d,\sigma^2).
\end{equation}
Given this variable $d_p$, we obtain the best-fit value of the theory parameter $c$ by minimising the $\chi^2$-statistic on the pseudodata replica:
\begin{equation}
c_p = \argmin_{\tilde{c}} \frac{\left(d_p - t(\tilde{c})\right)^2}{\sigma^2}.
\end{equation}
The resulting random variable $c_p$ can be multi-valued if there are multiple inequivalent minima. Calculus allows us to compute the minimum of the $\chi^2$-statistic in the one-dimensional case:
\begin{equation}
\frac{d}{d\tilde{c}} \chi^2(\tilde{c}) = -2t'(\tilde{c})(d_p - t(\tilde{c})) = 0,
\end{equation}
\noindent telling us that either $d_p = t(\tilde{c})$, or $t'(\tilde{c}) = 0$. To determine which are minima, we can compute a further derivative:
\begin{equation}
\frac{d^2}{d\tilde{c}^2} \chi^2(\tilde{c}) = -2t''(\tilde{c})(d_p - t(\tilde{c})) + 2(t'(\tilde{c}))^2.
\end{equation}
\noindent When $d_p = t(\tilde{c})$, the second derivative is positive, so this solution is always a minimum (when it exists). On the other hand, when $t'(\tilde{c}) = 0$, the second derivative is $-2t''(\tilde{c})(d_p - t(\tilde{c}))$. Depending on the signs of $t''(\tilde{c})$ and $d_p - t(\tilde{c})$ at this point, this solution can either be a minimum or a maximum. The cases are:
\begin{itemize}
\item $\tilde{c}$ is a minimum of $t$, so that $t''(\tilde{c}) > 0$. Then $\tilde{c}$ is a local minimum of the $\chi^2$-statistic if and only if $d_p < t(\tilde{c})$.
\item $\tilde{c}$ is a maximum of $t$, so that $t''(\tilde{c}) < 0$. Then $\tilde{c}$ is a local minimum of the $\chi^2$-statistic if and only if $d_p > t(\tilde{c})$.
\end{itemize}
In particular, if $\tilde{c}$ exists with $d_p = t(\tilde{c})$, then we have a \textit{global} minimum of the $\chi^2$. On the other hand, if this solution does not exist, continuity of the theory implies that we either have $t(\tilde{c}) < d_p$ for all $\tilde{c}$, or we have $t(\tilde{c}) > d_p$ for all $\tilde{c}$. \JM{This is only true on a finite domain, technically...}\\

Summarising, we see that:
\begin{equation}
c_p = \begin{cases} t^{-1}(d_p) & \text{if $d_p \in \textrm{im}(t)$,}\\[1.5ex] \end{cases}
\end{equation}
where $t^{-1}(d_p)$ is the preimage of the pseudodata $d_p$, and $(t')^{-1}(0)$ is the preimage of $0$ under the derivative (i.e. the stationary points of the theory).\\

Basic probability theory allows us to compute the distribution of $c_p$...

\begin{equation}
c_p \sim \int\limits_{as}^{as} dx\ \delta(c - t^{-1}(d_p)) \exp\left( -\frac{1}{2\sigma^2}(x - d)^2 \right)
\end{equation}


\subsection{Resolving the disagreement}
\label{subsec:resolution_in_1d}

Above, we have shown that the interval estimates produced by the frequentist, Bayesian and Monte-Carlo replica methods can disagree in the case of one data point and one theory parameter (although the methods do coincide for particularly simple theories $t(c)$, namely linear theories). However, there is no problem with this disagreement \textit{per se} - the interpretation of the intervals is different for each of the three methods.

This leaves open the question of which interval estimates are most useful. \\

The Monte-Carlo method can be used to reproduce both the frequentist confidence intervals and the Bayesian credible intervals in our toy model. In particular...\\

There are essentially three main approaches one may take to resolve the disagreement between the Bayesian 
method, whilst retaining a Monte-Carlo sampling approach:

\begin{enumerate}[label = (\roman*)]
\item Change the sampling distribution for the pseudodata replicas.
\item Change the loss function on which ...
\item Change the ...
\end{enumerate}





